Orbital shadowing, $\omega$-limit sets and minimality

Let $X$ be a compact Hausdorff space, with uniformity $\mathscr{U}$, and let $f \colon X \to X$ be a continuous function. For $D \in \mathscr{U}$, a $D$-pseudo-orbit is a sequence $(x_i)$ for which $(f(x_i),x_{i+1}) \in D$ for all indices $i$. In this paper we show that pseudo-orbits trap $\omega$-limit sets in a neighbourhood of prescribed accuracy after a uniform time period. A consequence of this is a generalisation of a result of Pilyugin et al: every system has the second weak shadowing property. By way of further applications we give a characterisation of minimal systems in terms of pseudo-orbits and show that every minimal system exhibits the strong orbital shadowing property.

==> Sections/Graveyard.tex <==
\begin{theorem}\label{thmMinimalStrong}
Let $X$ be a compact Hausdorff space. If $(X,f)$ is a minimal dynamical system then it exhibits the strong orbital shadowing property.
\end{theorem}
\begin{proof}
Let $E \in \mathscr{U}$ be given. Take $D \in \mathscr{U}$ and $n \in \mathbb{N}$ corresponding to $E$ as in Theorem \ref{thmOmega}. Now let $(x_i)_{i \geq 0}$ be a $D$-pseudo-orbit and take $z \in X$ such that
\[B_E\left(\{x_i\}^n _{i=0} \right) \supseteq \omega(z).\]
As $(X,f)$ is minimal $\omega(x)=X$ for any $x \in X$; in particular $\omega(z)=X$. It follows that
\[B_E\left(\{x_i\}^n _{i=0} \right)=X.\]
Since the $D$-pseudo-orbit $(x_i)_{i\geq 0}$ was picked arbitrarily, this holds for any $D$-pseudo-orbit. In particular, for any $N \in \mathbb{N}_0$
\[B_E\left(\{x_{N+i}\}^{n}_{i=0}\right) =X.\]
Furthermore, since every orbit sequence is a pseudo-orbit, for any $x \in X$ and any $N \in \mathbb{N}_0$, 
\[B_E\left(\{f^{N+i}(x)\}^{n}_{i=0}\right) =X.\]
The result follows.
\end{proof}

\begin{remark} We remark that in the course of the proof of Theorem \ref{thmMinimalStrong} we have actually proved a stronger property of minimal systems, that is: For any $E \in \mathscr{U}$ there exist $D \in \mathscr{U}$ and $n \in \mathbb{N}$ such that for any two $D$-pseudo orbits $(x_i)_{i \geq 0}$ and $(y_i)_{i \geq 0}$ 
\[\{y_i\}_{i =0} ^n \subseteq B_E\left( \{x_i\}_{i=0} ^n\right)\]
and
\[\{x_i\}_{i =0} ^n \subseteq B_E\left( \{y_i\}_{i=0} ^n\right).\]
In fact it is easy to verify that this property is also sufficient for a dynamical system to be minimal. Whilst we omit the proof of this sufficiency we formulate this result as Theorem \ref{thmMinimalIFF} below.
\end{remark}
